TDGIA:Effective Injection Attacks on Graph Neural Networks

Graph Neural Networks (GNNs) have achieved promising performance in various real-world applications. However, recent studies have shown that GNNs are vulnerable to adversarial attacks. In this paper, we study a recently-introduced realistic attack scenario on graphs -- graph injection attack (GIA). In the GIA scenario, the adversary is not able to modify the existing link structure and node attributes of the input graph, instead the attack is performed by injecting adversarial nodes into it. We present an analysis on the topological vulnerability of GNNs under GIA setting, based on which we propose the Topological Defective Graph Injection Attack (TDGIA) for effective injection attacks. TDGIA first introduces the topological defective edge selection strategy to choose the original nodes for connecting with the injected ones. It then designs the smooth feature optimization objective to generate the features for the injected nodes. Extensive experiments on large-scale datasets show that TDGIA can consistently and significantly outperform various attack baselines in attacking dozens of defense GNN models. Notably, the performance drop on target GNNs resultant from TDGIA is more than double the damage brought by the best attack solution among hundreds of submissions on KDD-CUP 2020.

==> 4.model.tex <==
\xz{We shall make this part more theoretical instead of being too practical}
In this section, we first proof the common flaw of GNN models under GIA. Aiming at this flaw, we design a general GIA approach that can be adapted to large-scale graphs. The GIA is based on a sequential injection scheme by applying edge selection and feature optimization consecutively.  

% \subsection{FGSM}
% \xz{Introduction of AFSGM and gradient based methods? How about Nettack?}
% The most straightforward method for adversarial attacks is Fast Gradient Sign Method(FGSM)\cite{goodfellow2014explaining}. It uses the gradients of a neural network to generate adversarial examples. The 

% \subsection{Sequential Injection Attack and AFGSM}
% As we separate the edge selection and feature optimization process for computational availability, deciding the number of links to be injected for each target node becomes a difficult task. We don't know whether the prediction of a node may alter or not before we optimize the feature of the injection nodes.

% More injection leads to higher confidence of success on attacking the target node, however when the injection node budget is limited, the assignment also needs to consider the efficiency of the attack. 

% The \textbf{sequential injection attack} method helps handle this. We inject new nodes in batches, and optimize them sequentially. If the prediction of a target node is already altered, we don't need to connect it to additional injection nodes. In each batch, the additional injection nodes are only connected to already altered nodes. i.e. Nodes in $\mathcal{N}_c$. 

% Both the optimization and sequential injection process needs an evaluater of how good the attack already is, in order to help them optimize features, or select edges for the new batch of injection nodes.  

% However, under the Black Box setting, the attacker doesn't have much information about the defensive model, except for the defensive model being some forms of GNNs. In this case, we build some surrogate GNN models in order to help evaluation during the injection of attack nodes. The attack is optimized using surrogate models, after the injection nodes are confirmed, the attack is then evaluated on test models. 

% The surrogate labels are not only helpful during the optimization and edge selection process, they're also used to estimate the labels of the nodes on test set since the true labels are not offered under the Black Box setting.

\subsection{Vulnerability of GNN Models under GIA}

We first investigate the vulnerability of GNN models under GIA. Note that not all models for node classification are GIA-attackable. If a model ignores the nodes or edges injected by GIA, the attack won't have any effect on it. For example, Multi-layer Perceptron (MLP), which ignores all edges on the graph and only classifies nodes according to node features, can not be affected by GIA. Because the injection nodes need to spread their information through edges to influence other nodes. It is important to identify the type of models that are vulnerable under GIA. We start with showing that a vast majority of GNN models are GIA-attackable.


% Now the problem raises-- which type of models $\mathcal{M}$ are GIA-attackable?

% \begin{definition}[Permutation Invariant]
% Let $\mathcal{M}:\mathbf{G}\rightarrow \{1,2,...,l\}^n$ be a GNN model that predicts the label for all nodes on the graph, it is Permuation Invariant, if for any $\mathbf{G}=(\mathbf{A},\mathbf{F}),\mathbf{G}'=(\mathbf{A}',\mathbf{F}')$ such that there exist a permuation of $1...n$, $(p_1,...,p_n)$, i.e. $\forall i,\mathbf{F}'_{p_i}=\mathbf{F}_i, \forall i,j, \mathbf{A}'_{p_ip_j}=\mathbf{A}_{ij}$, then $\forall i, \mathcal{M}(\mathbf{G}')_{p_i}=\mathcal{M}(\mathbf{G})_i$
% \end{definition}


\begin{definition}[Permutation Invariant]
Let $\mathbf{G}=(A, F)$ be an attributed graph with $n$ nodes. Let $\mathcal{M}:\mathbf{G}\rightarrow \{1,2,...,l\}^n$ be a model that predicts the labels for all nodes on $\mathbf{G}$. The model $\mathcal{M}$ is \textit{Permutation Invariant}, if for any $\mathbf{G}'=(\mathbf{A}',\mathbf{F}')$ such that $\mathbf{G}'$ is a permutation of $\mathbf{G}$, (i.e. there exists a permutation $\sigma$: $\{1, ..., n\} \rightarrow \{\sigma_1, ..., \sigma_n\}$, such that $\forall i\in\{1,2,...,n\}, \mathbf{F}'_{\sigma_i}=\mathbf{F}_i$ and $\forall (i,j)\in\{1,2,...,n\}^2, \mathbf{A}'_{\sigma_i\sigma_j}=\mathbf{A}_{ij}$), we have $\forall i\in\{1,2,...,n\}, \mathcal{M}(\mathbf{G}')_{\sigma_i}=\mathcal{M}(\mathbf{G})_i$.
\end{definition}


% \begin{definition}[GIA Attackable]

% Let $\mathcal{M}:\mathbf{G}\rightarrow \{1,2,...,l\}$ be a GNN model that predicts the label of node 0 on the graph. It is GIA-attackable, if there exist $\mathbf{G},\mathbf{G}'$, that 
% $\mathbf{G}$ is an induced subgraph of $\mathbf{G}'$, node $0$ in $\mathbf{G}'$ is still the same node 0 in $\mathbf{G}$, and that $\mathcal{M}(\mathbf{G})\neq \mathcal{M}(\mathbf{G}')$.

% \end{definition}
\begin{definition}[GIA-attackable]
The model $\mathcal{M}$ is GIA-attackable, if there exist two graphs $\mathbf{G_1}, \mathbf{G_2}$ containing the same node $i$, such that $\mathbf{G_1}$ is an induced subgraph of $\mathbf{G_2}$, and $\mathcal{M}(\mathbf{G_1})_i\neq \mathcal{M}(\mathbf{G_2})_i$.
\end{definition}

A model is GIA-attackable indicates that an attacker can change the prediction of a certain node $i$ by injecting nodes to the graph. For permutation invariant models, the positions of node $i$ in $\mathbf{G_1}, \mathbf{G_2}$ do not matter, since we can simply apply a permutation to change them to the same position. 

%A model is GIA-attackable indicates that the model may change the prediction of a node due to some injections, hence it is GIA-attackable. For permutation invariant models, whether the predicted label is for node 0 or other nodes does not matter, as we can simply use a permutation to permute any nodes to position 0 .

% \begin{definition}[Structural-Ignorant Model]
% \label{def:3}
% A structural-ignorant model is a model $\mathcal{M}:\mathbf{F}\rightarrow \{1,2,...,l\}$, which relies only on $\mathbf{F}$ for prediction, regardless of $\mathbf{A}$. i.e. $\forall \mathbf{A}_1,\mathbf{A}_2,\mathbf{F},\mathcal{M}(\mathbf{A}_1,\mathbf{F})=\mathcal{M}(\mathbf{A}_2,\mathbf{F})$. Clearly such a model is not GIA-attackable. 

% \end{definition}
\begin{definition}[Structural-Ignorant Model]
\label{def:3}
The model $\mathcal{M}$ is a structural-ignorant model, if $\forall \mathbf{G}_1=(\mathbf{A}_1,\mathbf{F}),\mathbf{G}_2=(\mathbf{A}_2,\mathbf{F})$, $\mathcal{M}(\mathbf{G}_1)_0=\mathcal{M}(\mathbf{G}_2)_0$. i.e. The model gives same predictions of node 0 based on same features. On the contrary, $\mathcal{M}$ is a non-structural-ignorant model, if there exist $\mathbf{G}_1=(\mathbf{A}_1,\mathbf{F}),\mathbf{G}_2=(\mathbf{A}_2,\mathbf{F})$,  $\mathbf{A}_1\neq\mathbf{A}_2$, $\mathcal{M}(\mathbf{G}_1)_0\neq\mathcal{M}(\mathbf{G}_2)_0$.
\end{definition}

% We prove that non-structural-ignorant models, i.e. models that rely on adjacency information for label prediction, are all GIA-attackable. If a model is not structural-ignorant, there exist $\mathbf{G}_1=(\mathbf{A}_1,\mathbf{F}),\mathbf{G}_2=(\mathbf{A}_2,\mathbf{F})$, $\mathbf{A}_1\neq\mathbf{A}_2$ $\mathcal{M}(\mathbf{G}_1)\neq\mathcal{M}(\mathbf{G}_2)$. 

% \begin{lemma}[Non-structural-ignorant Models are GIA-Attackable]

% Suppose $\mathcal{M}$ is permutation invariant model and not a structural-ignorant model, $\mathcal{M}$ is GIA-attackable.
% \end{lemma}
According to this definition, most GNNs are non-structural-ignorant, as they rely on structural information $\mathbf{A}$ for node classification instead of only using $\mathbf{F}$.

We then prove that non-structural-ignorant models are GIA-attackable.

\begin{lemma}[Non-structural-ignorant Models are GIA-Attackable]
\label{lemma:GIA}
If the model $\mathcal{M}$ is a non-structural-ignorant model and is permutation invariant, then $\mathcal{M}$ is GIA-attackable.
\end{lemma}


 \begin{proof}

 Combine the $\mathbf{G}_1$ and $\mathbf{G}_2$ mentioned above to a new graph $\mathbf{G}^{*}$ under the following way:

 We start from $\mathbf{G}^{*}=\mathbf{G}_1$, and add nodes from  $\mathbf{G}_2$ with index not being 0 to the graph. The added nodes maintain their features, have their index changed from $1...n-1$ to $n...2n-2$, and linked with each other according to their new index, except for their links with node 0, which is set to link node 0 in $\mathbf{G}^{*}$.

 Suppose $\mathcal{M}$ is not GIA-attackable, then
 \beq{
 \mathcal{M}(\mathbf{G}^{*})=\mathcal{M}(\mathbf{G_1}).
 }

 Then we apply the same process that we start from $\mathbf{G}^{**}=\mathbf{G}_2$, and add nodes from $\mathbf{G}_1$ with index not being 0 to the graph. Similarily we get 

 \beq{
 \mathcal{M}(\mathbf{G}^{**})=\mathcal{M}(\mathbf{G_2}).
 }

 As the model $\mathcal{M}$ being permutation invariant, while $\mathbf{G}^{*}$ and 
$\mathbf{G}^{**}$ are the same graph under permuation invariance, so 

\beq{
\mathcal{M}(\mathbf{G_2})=\mathcal{M}(\mathbf{G}^{**})=\mathcal{M}(\mathbf{G^{*}})=\mathcal{M}(\mathbf{G_1}).
 }

which contradicts to the initial assumption that $\mathcal{M}(\mathbf{G_1})\neq \mathcal{M}(\mathbf{G_2})$, so $\mathcal{M}$ is GIA-attackable.

\end{proof}


\hide{The proof of Lemma \ref{lemma:GIA} can be found in Appendix.} Therefore, we demonstrate that as long as a model is non-structural-ignorant, it is vulnerable against GIA attacks. 

% The effectiveness of GIA attacks still remains a question, and therefore our goal in this paper is to figure out effective and efficient ways to attack various GNN models.
\hide{
\subsection{Overview of Topological Defective Graph Injection Attack}

Aiming at the vulnerability of GNN models under GIA, we propose Topological Defective Graph Injection Attack (\name), which can effectively decrease the performance of GNN models on large-scale graph through node injection. The overview of \name is illustrated in ~\figurename~\ref{}. In the black-box scenario, we do not direct access to the target model. Thus, we first train a surrogate model for the same node classification task. Then, we inject vicious nodes to attack the surrogate model and transfer them to the target model. 

Different from previous works that jointly optimize connections and attributes on the graph, \name separate the process of edge and feature optimization. The reason is that for large real-world graphs like Aminer~\cite{tang2016aminer}, we need a more efficient solution rather than optimization in a huge search space. First, according to topological properties of the graph, we inject vicious nodes and identify defective edges that are most likely to perturb the predictions of GNN models. Second, we optimize the features of injected nodes by a newly proposed loss function. 


\qinkai{
Add a figure to illustrate the entire process of \name.
}
}
% \subsection{Separation of Edge and Feature Optimization}
% Though Nettack-like joint optimization method works for small graphs, for large, real-world graphs like Aminer\cite{tang2016aminer}, the cost of joint optimization on edges and features is unacceptable. A cost-efficent solution is to separate the process of edge and feature optimization. We first select the edges that are likely to make the largest perturbations on GNN model predictions, then we optimize features accordingly. 

\subsection{Topological properties of a GNN layer}
\xz{ My suggestion on arrangement: 1: start with layer, 2: attack based on layer 3: expand the layer logic to full GNN models}
\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{generalgnnlayer}
    \caption{Illustration of a general GNN layer.}
    \label{fig:general}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{TDGIA}
    \caption{Illustration of the proposed TDGIA framework}
    \label{fig:general}
\end{figure}
% As our target is to attack GNNs, GNNs is usually a stack of information propagation, that is, on a network, it aggregates and updates node features iteratively with \cite{xu2018powerful}

\hide{
Our idea is to harness the topology of graph to design an adversarial attack, we first explore the topological properties of GNN models. GNN is usually a stack of information propagation~\cite{xu2018powerful}, which aggregates and updates node features iteratively with 
}

Despite there exists dozens of variations, generally a GNN layer can be represented as the following.

\beq{
\label{eqn:agg}
\mathbf{h}_{v}^{k}=\phi(\mathbf{h}_v^{k-1},\mathbf{f}(\mathbf{h}_u^{k-1},u\in \mathcal{N}(v))),
}
where $\phi,\mathbf{f}$ are vector-valued functions and $\mathcal{N}(v)$ is the neighborhood of node $v$, while $\mathbf{h}_{v}^{k}$ being the representation of node $v$ at layer $k$. $\mathbf{h}_{v}^{0}$ is the input feature of node $v$ while $\mathbf{h}_{v}^{f}$ is the final output that decides its label.

The neighborhood $\mathcal{N}(v)$ may include nodes that are directly linked to $v$, as well as nodes that can be connected to $v$ within a radius of $2,3...$. To make it clear, suppose we use $\mathcal{A}_{t}(v)$ to represent the $t-degree$ neighbors of $v$, (nodes that can reach $v$ with a path with length being exactly $t$), equation \ref{eqn:agg} can be expressed more clearly by

\beq{
\begin{split}
\mathbf{h}_{v}^{k}=&\phi(\mathbf{f}_0(\mathbf{h}_v^{k-1}),\mathbf{f}_1(\mathbf{h}_u^{k-1},u\in \mathcal{A}_{1}(v)),\mathbf{f}_2(\mathbf{h}_u^{k-1},u\in \mathcal{A}_{2}(v)),\\&...,\mathbf{f}_n(\mathbf{h}_u^{k-1},u\in \mathcal{A}_{n}(v))).
\end{split}
}

\xz{Seems hard to describe this} \qinkai{Can we define small changes from the graph level to avoid discussion of each $\mathcal{A}_n$?}
Suppose we change the graph by a little so that $\mathcal{A}_1,...\mathcal{A}_n$ changes by $\Delta \mathcal{A}_1,...\Delta \mathcal{A}_n$ and $\mathbf{f}_0,...\mathbf{f}_n$ changes by a comparable small amount,
\beq{
\begin{split}
\mathbf{h}_{v}'^k= &\mathbf{h}_{v}^k+\frac{\partial\phi}{\partial \mathbf{f}_0}(\mathbf{f}_0'-\mathbf{f}_0)+\frac{\partial \phi}{\partial \mathbf{f}_1}(\mathbf{f}_1'-\mathbf{f}_1)+...+\frac{\partial \phi}{\partial \mathbf{f}_n}(\mathbf{f}_n'-\mathbf{f}_n)\\&+O((\Delta \mathbf{f}_0)^2+(\Delta \mathbf{f}_1)^2+...+(\Delta \mathbf{f}_n)^2))
\end{split}
}

We take $\frac{\partial \phi}{\partial \mathbf{f}_i}$ at layer $k$ to be $\mathbf{p}_{ik}$, then 

\beq{
\mathbf{h}_{v}'^k-\mathbf{h}_v^k=\sum_{j=0}^{n}\mathbf{p}_{jk}\Delta \mathbf{f}_j+o(\sum_j\Delta \mathbf{f}_j)
}


Suppose $\mathbf{f}$ is a form of weighted averaging, which is also the case for most of the GNNs. \xz{this is an assumption!} \qinkai{Maybe we can assume this is an aggregation/MLP function to make it more general.}
\beq{
\mathbf{f}_i=\sum_{u\in \mathcal{A}_i(v)} w_{u,i}\mathbf{h}_u^{k-1}, w_{u,i}=\psi_i(u)
}
where $\psi_i(u)$ is a function that only correspond to the property of node $u$.
Then 

\beq{
\Delta \mathbf{f}_j=\sum_{u\in \mathcal{A}'_i(v)\bigcup \mathcal{A}_i(v)}(\Delta w_{u,i}\mathbf{h}_u+w_{u,i}\Delta \mathbf{h}_u)
}

\xz{We put "defective edge selection" here.}


Here, we suppose $\Delta w_u=w'_u-w_u, \Delta \mathbf{h}_u=h'_u-\mathbf{h}_u$ if $u\in \mathcal{A}'_i(v)$ and $u\in \mathcal{A}_i(v)$, for $u\in \mathcal{A}'_i(v),u\notin\mathcal{A}_i(v)$, $\Delta w_u=w'_u, \Delta \mathbf{h}_u=h'_u$, for $u\notin \mathcal{A}'_i(v),u\in\mathcal{A}_i(v)$, $\Delta w_u=-w_u, \Delta \mathbf{h}_u=-\mathbf{h}_u$.

Therefore,

\beq{
\Delta \mathbf{h}_{v}^k=\sum_{i=0}^{n}\mathbf{p}_{ik}\sum_{u\in \mathcal{A}'_i(v)\bigcup \mathcal{A}_i(v)} (\Delta w_u\mathbf{h}_u^{k-1}+w_u\Delta \mathbf{h}_u^{k-1})
}

\beq{
\Delta \mathbf{h}_{v}^k=\sum_i\sum_{u\in \mathcal{A}'_i(v)\bigcup \mathcal{A}_i(v)} (\Delta w_{u,i}\mathbf{p}_{ik}\mathbf{h}_u^{k-1}+w_{u,i}\mathbf{p}_{ik}\Delta \mathbf{h}_u^{k-1})
}

Now let's consider multiple layers. Suppose $\Delta \mathbf{h}_v^k$ can be expressed in the following form,

\beq{
\label{ini}
\Delta \mathbf{h}_{v}^k=\sum_i\sum_{u\in \mathcal{A}'_i(v)\bigcup \mathcal{A}_i(v)} (\Delta w_{u,i}\sum_{l=1}^{k}\mathbf{p}_{il}\mathbf{h}_u^{l-1}+w_{u,i}\mathbf{p}_{ik}\Delta \mathbf{h}_u^{0})
}

Where $p$ is a formatting variable and \xz{How to describe this? This $p$ is not the same as the previous one.}. For $k=1$ obviously it holds. Then
\beq{
\begin{split}
\Delta \mathbf{h}_v^{k+1}=\sum_i\sum_{u\in \mathcal{A}'_i(v)\bigcup \mathcal{A}_i(v)} (\Delta w_{u,i}\mathbf{p}_{ik+1}\mathbf{h}_u^{k}+w_{u,i}\mathbf{p}_{ik+1}\Delta \mathbf{h}_u^{k})\\
=\sum_i\sum_{u\in \mathcal{A}'_i(v)\bigcup \mathcal{A}_i(v)} (\Delta w_{u,i}\mathbf{p}_{ik+1}\mathbf{h}_u^{k}+\\
w_{u,i}\mathbf{p}_{ik+1}\sum_j\sum_{t\in \mathcal{A}'_j(u)\bigcup \mathcal{A}_j(u)} (\Delta w_{t,j}\sum_{l=1}^{k-1}\mathbf{p}_{jl}\mathbf{h}_u^{l}+w_{t,j}\mathbf{p}_{jk}\Delta \mathbf{h}_u^{0})\\
=\sum_i\sum_{u\in \mathcal{A}'_i(v)\bigcup \mathcal{A}_i(v)} (\Delta w_{u,i}\sum_{l=1}^{k}p'_{il}\mathbf{h}_u^{l}+w_{u,i}p'_{ik+1}\Delta \mathbf{h}_u^{0})
\end{split}
}

Which $p'$ is a function of the previous $p$s.  

Therefore, \xz{needs more clarification}

\beq{
\label{deltah}
\Delta \mathbf{h}_{v}^f=\sum_i\sum_{u\in \mathcal{A}'_i(v)\bigcup \mathcal{A}_i(v)} (\Delta w_{u,i}\sum_{l=1}^{f}\mathbf{p}_{il}\mathbf{h}_u^{l-1}+w_{u,i}\mathbf{p}_{ik}\Delta \mathbf{h}_u^{0})
}

And when we have $w_{u,i}=0,\forall u\notin \mathcal{G}$ for GIA, and assuming $\Delta w_{u,i}<<1$, the function becomes

\beq{
\label{attackrule}
\Delta \mathbf{h}_{v}^f=\sum_i\sum_{u\in \mathcal{A}'_i(v)\bigcup \mathcal{A}_i(v)} \Delta w_{u,i}\sum_{l=1}^{f}\mathbf{p}_{il}\mathbf{h}_u^{l-1}
}

For a model, $\mathbf{p}_{il}$ and $\mathbf{h}_u^{t}$ might not be revealed until we finish our optimization. However, $w_{u,i}$ is commonly pre-defined by edges or other factors of the graph. For example, in GCN, a single layer 
$w_{u_i}=\frac{1}{\sqrt{deg(u)deg(v)}}\delta(i,1)$, where $\delta(a,b)=1,a=b,0,a\neq b$

\xz{ Is it really needed?}

\subsection{Defective Edge Selection}

\qinkai{
With previous exploration on the topological properties of GNN models, we propose defective edge selection, which selects edges for injected nodes that maximize the perturbation of GNN's output.  
}

What the attacker is trying to do is to guide the model to behave wrongly. It is not necessarily but better to maximize $\sum\Delta \mathbf{h}_v, v\in C$, where $C$ is the node set that the model still produces a correct result, i.e. nodes that still need attack.

As we need to select edges before optimizing features for injected nodes, from equation \ref{attackrule}, our idea is that, the larger scale of $\Delta w_{u,i}$, we might get a larger shift on $\Delta \mathbf{h}_v$.

For GIA, as it only injects new nodes and not removing any existing nodes of edges, we have $\forall v,i, \mathcal{A}_i(v)\subseteq\mathcal{A}'_i(v)$. We take $w^*_{u,i}=\frac{w_{u,i}}{\sum_{u\in \mathcal{A}'_i(v)w_{u,i}}}$, as the normalized weight of each node for $i^{th}$-level neighborhood of node $v$. \qinkai{Definition of $\mathcal{A'}$ is different from the previous one.}

\beq{
\sum_{u\in \mathcal{A}'_i(v)}|\Delta w^*_{u,i}|\geq 2r_{v,i}=2\sum_{\mathcal{A}_{i}(v)} w^*_{u,i}
}

Here $r_n$ is the proportion of weights of newly added nodes for $i^{th}$-level neighborhood after GIA. 

We take the assumption that GNNs usually care more about near neighbors when $i$ being small, instead of faraway neighborhoods when $i$ being large. So in our attempt we first maximize $\sum_{v\in C}r_{v,1}$ and then maximizing the second-level perturbations. \qinkai{Not convincing. Need a quantitative explanation that explain superiority of the first-level perturbations.}



\vpara{Maximization of level-1 perturbation}
We start from common $w_{u,i}$ functions used in GNNs. Following GCN\cite{kipf2016semi}, various types of GNNs use 
\beq{
\label{eqn:w1}
w_{u,1}=\frac{1}{\sqrt{deg(u)deg(v)}}
}. For methods based on the mean-pooling of GraphSAGE\cite{hamilton2017inductive}, 
\beq{
\label{eqn:w2}
w_{u,1}=\frac{1}{deg(v)}
}is used. For GAT\cite{velivckovic2018graph} and other attention-based methods, $w_{u,1}$ may be based on the softmax of the attention score of $\mathbf{h}_u^l$. Most of these ways to generate $w_{u,1}$ only incorporates the feature or degree information of node $u$ and $v$, and does not correlate to $w_{t,i},t\neq u$. That is to say, we can separate $\sum_{u\in \mathcal{A}_1(v)\backslash\mathcal{A}_1(v)} w_{u,1}$ and $\sum_{u\in \mathcal{A}_1(v)} w_{u,1}$. 

Take $c_1=\sum_{u\in \mathcal{A}_1(v)\backslash\mathcal{A}_1(v)} w_{u,1}$, and $c_2=\sum_{u\in \mathcal{A}_1(v)} w_{u,1}$, then $r_{v,1}=\frac{c_1}{c_1+c_2}=\frac{1}{1+\frac{c_2}{c_1}}$, given $c_1$ does not change due to $c_2$, this suggests us that, to make $\sum r_{v,1}$ large, the injected nodes shall be connected to nodes with $\lambda=\frac{c_1}{c_2}$ being large. Here $c_2$ can be approximated using equation \ref{eqn:w1} and \ref{eqn:w2}. 
\xz{needs refinement}

\xz{After Conducting a lot of experiments, now I think random is not worse than this level-2 link assignment being assigned... 61.21(this one) vs 61.38(random)}
\vpara{Maximization of level-2 perturbation}
\xz{maximizing level-1 and level-2 perturbation follows different logic, which is hard to describe.}
Suppose we're already maximizing $\sum_{v\in C}r_{v,1}$ by assigning the injection nodes to nodes in $C$ with minimal $c_2$.

As every injection node may be limited to a certain number of links to avoid being detected and removed by defense methods, assigning those links still remain a question, as two nodes that are linked to the same injection node becomes second-level neighbors of each other, and start to influence the embeddings of each other.

We start from maximizing $\sum_{v\in C} r_{v,2}$, still it's better to add neighbors to those nodes with a small $c_2=\sum_{u\in \mathcal{A}_2(v) w_{u,2}}$, however that is already achieved in the level-1 perturbation part. 

Recall equation (\ref{attackrule}),

\beq{
\Delta \mathbf{h}_{v}^f=\sum_i\sum_{u\in \mathcal{A}'_i(v)} \Delta w_{u,i}\sum_{l=1}^{f}\mathbf{p}_{il}\mathbf{h}_u^{l-1}
}

For $i=2$, we tend to maximize the scale of 

\beq{
\Delta \mathbf{h}_{v}^\mathbf{f}(2)=\sum_{u\in \mathcal{A}'_2(v)} \Delta w_{u,2}\sum_{l=1}^{f}\mathbf{p}_{2l}\mathbf{h}_u^{l-1}
}

\xz{ This is just a logical way, needs refinement on this expression}
Different from newly injected nodes whose embeddings are easy to adjust, for level-2 perturbation, the nodes that newly appear in second-level neighborhood are usually nodes that are linked together by an injection node. And their $\mathbf{h}_u$ are fixed as we cannot change features of existing nodes in GIA. 

This means it is better to make the newly-introduced nodes far-away from the original representation. That is to say, we shall let 

\beq{
\begin{split}
d_1=\frac{\sum_{u\in A_2(v)}  w_{u,2}\sum_{l=1}^{f}\mathbf{p}_{2l}\mathbf{h}_u^{l-1}}{\sum_{u\in  A_2(v)}w_{u,2}}
\\d_2=\frac{\sum_{u\in \mathcal{A}'_2(v)\backslash A_2(v)}  w_{u,2}\sum_{l=1}^{f}\mathbf{p}_{2l}\mathbf{h}_u^{l-1}}{\sum_{u\in \mathcal{A}'_2(v)\backslash A_2(v)}w_{u,2}}
\end{split}
}

be as different as possible. Which means for GIA it's more efficient to link nodes with different $\mathbf{h}_u^{l}$ to the same injection node. That is to say, make $||d_1-d_2||$ as large as possible. 


\subsection{Smooth Adversarial Optimization}

\qinkai{
After the defective edges selection, it is necessary to optimize the features of injected nodes. We design a new loss function 
}

Given a model $\mathcal{M}$, an adjacency matrix $\mathbf{A}'$ including the selected edges of injection nodes, features of the nodes on the original graph $\mathbf{F}$, we wish to find a way to optimize $\mathbf{F}^*$, the features of injected nodes, to attack the model prediction $\mathcal{M}(\mathbf{A}',\mathbf{F},\mathbf{F}^*)$.

\vpara{Smooth Loss Function}
According to section \ref{sec:FGSM}\xz{need background from  I guess}, in FGSM, we optimize the inverse of cross entropy loss, which is to minimize
\beq{
loss(\mathcal{L}_{predict},\mathcal{L}_{train})=-D_{KL}(\mathcal{L}_{predict}||\mathcal{L}_{train})=E[log(\mathbf{p}_{correct})],
}
where $\mathbf{p}_{correct}$ is predicted probability for the correct label. 

Simply setting this loss may cause gradient explosion, as 

\beq{
\frac{\partial log p}{\partial p}=\frac{1}{p},
}
which goes to $\infty$ as $p\rightarrow 0$. To alter this, we change the loss function to 

\beq{
loss(\mathcal{L}_{predict},\mathcal{L}_{test})=E[min(r+log(\mathbf{p}_{correct}),0)^2],
}

where $r$ is a set boundary. Therefore the derivative becomes

\beq{
\frac{\partial l}{\partial p}=\left\{
\begin{split}
\frac{2\sqrt{l}}{p},l>0 \\ 0,l=0
\end{split}\right
}

Therefor $\frac{\partial l}{\partial p}\rightarrow 0$ when $l\rightarrow 0$, and the optimization becomes stable.

\vpara{Smooth Feature Optimization}
In GIA, there's usually a constraint on the range of feature of the injection nodes. The defenders may also establish criteria to filter out abnormal features. Hence we need to limit the range of the features of the injection nodes. 

The simplest way is to use clamp during optimization. In the optimization stage we on raw features but do a clamp before feeding the features into the model, and after optimization we output the clamped features as injection features.
\beq{
Clamp(x,min,max)=\left\{\begin{split}min,x<min\\ x,min<x<max\\max,x>max\end{split}\right
}

However, this leads to zero gradient if $x$ exceeds the maximal or minimal threshold, $x$ will then be fixed at maximal or minimal, despite the change of features of other nodes or dimensions. This reduces the effectiveness of optimization.

In order to smooth this process, we adopt a smooth process. To map a real number onto $(min,max)$ smoothly, we use a sin function for injection feature optimization:

\beq{
smoothmap(x,min,max)=\frac{min+max}{2}+\frac{max-min}{2} sin(x).
}

In the optimization stage we on raw features but do $smoothmap$ before feeding the features into the model, and after optimization we output the $smoothmap$ features as injection features.
\xz{need to refine word representation of this}


\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{howgiawork.png}
    \caption{How GIA work on a GNN layer.}
    \label{fig:gia}
\end{figure}

%\subsection{C & S}

\begin{algorithm}[t]
\SetAlgoLined
\KwResult{injection nodes $\mathcal{N}^{+}$, links of the injection nodes $\mathcal{E}^{+}$, features of the injection nodes $\mathcal{F}^+$}
 Given training set labels $\mathcal{L}_t$, graph $\mathcal{G}=\{\mathbf{A},\mathbf{F}\}$, injection node budget $b$, degree budget for each node $d$;
 
 Train surrogate models $\mathcal{M}$ , generate estimation labels $\mathcal{L}'$. 
 
 Initialize iteration count $i=0$.
 
 \While{$b>0$}{
  $i=i+1$, set up $k_i\leq b$, number of nodes to be injected in this iteration.
  
  $\forall n\in \mathbf{T}$, calculate $p(n\in C)$ using $\mathcal{M}$. 
  
  Calculate aggregation weight factor $\lambda$ for each node $n$.
  
  Select top $kc$ nodes with highest value $\mu(p,\lambda)$.
  
  Assign the $d$ injection nodes to link the $k_id$ candidate nodes to be linked, using their estimation labels $\mathcal{L}'$. 
  
  Initialize $\mathcal{F}_i^+$ randomly, optimize $\bigcup\mathbf{p}_{j\leq i}\mathcal{F}_{j}^{+}$ with smooth feature optimization. 
  
  Update $b_i=|\mathcal{N}_i^+|,b=b-b_i,\mathcal{N}^+=\bigcup\mathcal{N}_i^+,\mathcal{E}^+=\bigcup\mathcal{E}_i^+,\mathcal{F}^+=\bigcup\mathcal{F}_i^+$
  
  Update the current graph
  $\mathcal{N}'=\mathcal{N}\oplus\mathcal{N}^+,\mathcal{E}'=\mathcal{E}\oplus\mathcal{E}^+,\mathcal{F}'=\mathcal{F}\oplus\mathcal{F}^+,\mathcal{G}'=\{\mathcal{N}',\mathcal{E}',\mathcal{F}'\}$
 }
 Combine nodes added from all iterations. $\mathcal{N}^+=\bigcup\mathbf{p}_i\mathcal{N}_i^+,\mathcal{E}^+=\bigcup\mathbf{p}_i\mathcal{E}_i^+,\mathcal{F}^+=\bigcup\mathbf{p}_i\mathcal{F}_i^+$
 \caption{Topological Defective Graph Injection Attack (\name)}
 %\vspace{-0.1in}
 \label{algo:bb}
 %\vspace{-0.1in}
\end{algorithm}

==> 5.exp.tex <==
%\xz{Time complexity in 5.2--Summary}
\subsection{Datasets}
We conduct our experiments on three large-scale public datasets, including 
1) the KDD-CUP dataset\footnote{https://www.biendata.xyz/competition/kddcup\_2020\_formal/}, a large-scale citation dataset used in KDD-CUP 2020 \textit{Graph Adversarial Attack \& Defense} competition, 
2) ogbn-arxiv~\cite{hu2020open}, a benchmark citation dataset, 
and
3) Reddit~\cite{hamilton2017inductive}, an online forum post dataset. 
Statistics of these datasets and our set injection constraints are displayed in Table \ref{tab:datasets}. 
Additional details of datasets are covered in Appendix \ref{app:repro}.

% For ogbn-arxiv and Reddit we evaluate our attacks on 7 representative defense models, while for KDD-CUP the evaluation is based on 12 best candidate defense submissions provided in the dataset. 

\begin{table*}[t]
\small
  \centering
  \caption{\label{tab:match_stats} Statistics of datasets. We consider only unique undirected edges.}
%   \renewcommand{\arraystretch}{1.2}
  \begin{tabular}{|c|r|r|r|r|r|c|c|c|c|c|c|}
    \hline \hline
    \multirow{2}*{Dataset} &\multirow{2}*{Nodes} & \multirow{2}*{\makecell{Train\\ nodes}} & \multirow{2}*{\makecell{Val \\nodes}} & \multirow{2}*{\makecell{Test\\ nodes}} & \multirow{2}*{Edges} & \multirow{2}*{Features} & \multirow{2}*{Classes} & \multirow{2}*{\makecell{Feature \\range}} & \multirow{2}*{\makecell{Injection\\feature range}} & \multirow{2}*{\makecell{Injected \\ nodes}} & \multirow{2}*{\makecell{Injection \\ degree limit}}\\
    &&&&&&&&&&&\\
    \hline
    KDD-CUP & 659,574 & 580,000 & 29,574 & 50,000 & 2,878,577 & 100 & 18 & -1.74$\sim$1.63 & -1$\sim$ 1 & 500 &100\\
    ogbn-arxiv & 169,343 & 90,941 & 29,799 & 48,603 & 1,157,799 &128 & 40 & -1.39$\sim$1.64 & -1$\sim$1 & 500 &100\\
    Reddit & 232,965 & 153,932 & 23,699 & 55,334 & 11,606,919 & 602 & 41 & -0.27$\sim$0.26 & -0.25$\sim$0.25 & 500 & 100\\
    \hline \hline
  \end{tabular}
  \label{tab:datasets}
\end{table*}
\begin{table}[t]
\small
    \centering
    \caption{ Performance(\%) of different GIA methods on KDD-CUP dataset over 12 top KDD-CUP defense submissions. Best results are bolded. }
    
    \label{tab:kddcup}
    % \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline \hline
       & \multirow{2}*{\makecell {Attack\\ Method}} & \multirow{2}*{\makecell {Average \\Accuracy}} & \multirow{2}*{\makecell{Top-3\\ Defense}} & \multirow{2}*{\makecell{Weighted\\Average}} &  \multirow{2}*{Reduction} \\
       &&&&&\\
       \cline{1-6}
      Clean & - & 65.54 & 70.02 & 68.57 & -\\
       \hline
       %&NTTDOCOMO LABS& 52.00$\pm$0.97 & 13.91\%\\
      %& ADVERSARIES & 44.85$\pm$1.39 & 25.91\%\\
      % & DeepBlueAI & 42.14$\pm$3.10 &30.23\%\\
      % & cccn & 52.01$\pm$0.97 \\
      \multirow{5}*{\makecell{ KDD-CUP\\Top-5 \\ Attack \\ Submissions}}  & advers& 63.44 &68.85 &67.09 & 1.48\\
       & dafts & 63.91 &68.50 & 67.02 & 1.55 \\
       &ntt &60.21 & 68.80 & 66.27 & 2.30 \\
       %& SPEIT-submission & 61.97 & 69.49 & 67.32 & 1.25\\
&simong   & 60.02     &    68.59  &       66.29 & 2.28\\
&u1234 &     61.18     &          67.95 &  64.87 & 3.70\\
       \hline
        \multirow{3}*{\makecell{Baseline \\Methods}}&FGSM & 59.80 & 67.44 & 65.04 & 3.53 \\
      %  &FGSM(use sin)& 58.49 & 67.09 & 64.44 & 4.13\\
      & AFGSM & 59.22 & 67.37 & 64.74 & 3.83\\
%       & AFGSM(use sin) & 58.43 & 67.05 & 64.39 & 4.18\\
       & SPEIT & 61.89 & 68.16 & 66.13 & 2.44 \\
      % & Best of Above & 59.22 & 67.37 & 64.74 & 3.83\\
       \hline
       \model &\model & \textbf{55.00} & \textbf{64.49} & \textbf{60.49} & \textbf{8.08} \\
      % \cline{2-6}
       
      % &Mixed& \textbf{54.80}&65.73 & 61.04 & 7.53 \\
      % & \multicolumn{5}{c|}{\xz{Shall we remove the "mixed"? It seems that mixed attack is worse than attack only on GCN}}\\
        \hline \hline
    \end{tabular}
   \vspace{-0.15in}
\end{table}

\begin{table}[t]
\small
    \centering
    \caption{ Performance(\%) of different GIA methods on Reddit and ogbn-arxiv dataset over 7 representative defense models. Best results are bolded.}
    
    \label{tab:reddit}
    % \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline \hline
       \multirow{2}*{Dataset}& \multirow{2}*{\makecell {Attack\\ Method}} & \multirow{2}*{\makecell {Average \\Accuracy}} & \multirow{2}*{\makecell{Top-3\\ Defense}} & \multirow{2}*{\makecell{Weighted\\Average}} &  \multirow{2}*{Reduction} \\
       &&&&&\\
       \cline{1-6}
      \multirow{5}*{Reddit} & Clean & 94.86 & 95.94 & 95.62 & -\\
       \cline{2-6}
       %&NTTDOCOMO LABS& 52.00$\pm$0.97 & 13.91\%\\
      %& ADVERSARIES & 44.85$\pm$1.39 & 25.91\%\\
      % & DeepBlueAI & 42.14$\pm$3.10 &30.23\%\\
      % & cccn & 52.01$\pm$0.97 \\
     
       \cline{2-6}
        &FGSM& 92.26 & 94.61 & 93.80 & 1.82\\
       & AFGSM & 91.46 & 94.64 & 93.61 & 2.01\\
       & SPEIT & 93.35 & 94.27 & 93.99 & 1.63\\ 
       
       \cline{2-6}
       
       &\model & \textbf{86.11} & \textbf{88.95} & \textbf{88.14} & \textbf{7.48} \\
       \hline
       \multirow{5}*{ogbn-arxiv} & Clean & 70.86 & 71.61 & 71.34 &  -\\
       \cline{2-6}
       %&NTTDOCOMO LABS& 52.00$\pm$0.97 & 13.91\%\\
      %& ADVERSARIES & 44.85$\pm$1.39 & 25.91\%\\
      % & DeepBlueAI & 42.14$\pm$3.10 &30.23\%\\
      % & cccn & 52.01$\pm$0.97 \\
     
       \cline{2-6}
       &FGSM&66.40 & 69.57 & 68.62 & 2.72 \\
       & AFGSM & 62.60 & 69.08 & 66.96 & 4.38\\
       & SPEIT & 66.93 & 69.56 & 68.63 & 2.71 \\ 
     
       \cline{2-6}
       &\model & \textbf{57.00} & \textbf{59.23} & \textbf{58.53} & \textbf{12.81}  \\
        \hline \hline
    \end{tabular}
   \vspace{-0.15in}
\end{table}

\subsection{The GNN Models}
\label{sec:base}
\vpara{Surrogate Attack Model.}  GCN~\cite{kipf2016semi} is the most fundamental and most widely-used model among all GNN variants. Vanilla GCNs are easy to attack~\cite{zugner2018adversarial,wang2020scalable}. However, when incorporated with LayerNorm~\cite{ba2016layer}, it becomes much more robust, and therefore is used by some top-competitors in KDD-CUP and achieved good defense results. In our experiments, we mainly use GCN as the surrogate model to conduct transfer attacks. We use GCNs (with LayerNorm) with 3 hidden layers of dimension 256, 128, 64 respectively. Following the black-box setting, we first train the GCN model, perform \model on it, and transfer the attack to all defense methods. 

\vpara{Defense Models.} For KDD-CUP dataset,  it offers 12 best defense submissions (including models and weights), which are considered as defense models. For Reddit and ogbn-arxiv datasets, we re-implement the 7 most representative GNN models (also appeared in KDD-CUP submissions), GCN~\cite{kipf2016semi}, SGCN~\cite{wu2019simplifying}, TAGCN~\cite{du2017topology}, GraphSAGE~\cite{hamilton2017inductive}, RobustGCN~\cite{zhu2019robust}, GIN~\cite{xu2018powerful} and APPNP~\cite{klicpera2018predict} as defense models. We train these models on the original graph and fix them for defense evaluation against GIA methods.
Details of these models are listed in Appendix \ref{app:models}.

\subsection{Evaluation Metric}
To evaluate GIA methods, we consider both the performance reduction and the generalization ability. Our evaluation is mainly based on the weighted average metric proposed in KDD-CUP dataset. The metric attaches a weight to each defense model based on its robustness under GIA, i.e. more robust defense gets a higher weight. This encourages the adversary to focus on generalization ability throughout all defense models, and to design more general attacks.

In addition to weighted average, we also provide the average accuracy among all defense models, and that of the Top-3 defense models. The three evaluation metrics are formulated below:

Suppose $s_1,s_2,...s_n$ are $n$ sorted accuracy scores of $n$ different defense GNN models against a GIA attack, $s_1\geq s_2\geq s_3...\geq s_n$. 
\beq{
s_{avg}=\frac{1}{n}\sum_{i=1}^{n}s_i,
}
\beq{
s_{top3}=\frac{1}{n}\sum_{i=1}^{3}s_i,
}
\beq{
\label{eqn:w}
s_{weight}=\sum_{i=1}^{n}w_is_i, \sum_{i=1}^{n}w_i=1, w_1\geq w_2\geq ... \geq w_n.
}

For KDD-CUP we use the weight $w$ given in the dataset, for ogbn-arxiv and Reddit, we set the weights ourselves. See Appendix \ref{app:repro} for details.

\subsection{Baseline Attack Methods}
\vpara{Baseline Attack Methods.} We compare our \model approach with different baselines, including 
FGSM~\cite{szegedy2013intriguing}, 
AFGSM~\cite{wang2020scalable}, 
the top five attack submissions of KDD-CUP 2020, 
and the SPEIT method~\cite{zheng2020kdd}, which is the attack method used by the champion team (as measured by both attack and defense) of KDD-CUP 2020. 
Note that NIPA~\cite{sun2020adversarial} covered in Table~\ref{tab:diffs} is not scalable enough for the large-scale datasets we use.

%\yx{to explain why NINA in Table 1 is not used as baseline}

 %\yx{don't understand 'than training the gnn model'}
%\hide{%====================================================================
Specifically, FGSM and AFGSM are adapted to the GIA settings with black-box and evasion attacks.
%We consider FGSM and AFGSM.
Inheriting from the original idea of Fast Gradient Sign~\cite{szegedy2013intriguing}, we randomly connect injected nodes to the target nodes, and optimize their features with inverse KL divergence. (Eq. \ref {eqn:loss})
AFGSM offers an improvement of FGSM, which captures the additive property of node injection. 
In AFGSM, the newly injected node may be better optimized when considering previous ones. 
We inherit this idea of sequential injection and apply it to the GIA settings. %However, the feature-edge-joint-optimization process in original AFGSM can't deal with large-scale graphs considered in this paper. We adapt it to the two-step process.  
%}%end 0f hide====================================================================


\vpara{Experimental Settings.} For each dataset, we set up the upper limit of 500 injected nodes and 100 degree for each injected node during injection generation. The feature limit is set according to the range of features in the dataset (Cf Table \ref{tab:datasets}).

For experiments on KDD-CUP dataset, despite the degrees limit for each injected node being 100, most submitted defense methods include some forms of filter processes that filters out nodes according to degrees. Therefore, in our experiments, we apply an artificial limit of 88 to avoid being filtered out. The limit is applied to both \model and the baseline methods. The reproducibility details are introduced in Appendix \ref{app:repro}.

\subsection{Performance of \model}

The performance of \model on KDD-CUP dataset is illuastrated in Table \ref{tab:kddcup}, while the results for Reddit and ogbn-arxiv are shown in Table \ref{tab:reddit}. As can be seen,  \model significantly outperforms all baseline methods by a large gap, more than doubling the reduction on weighted average for all three datasets, suggesting that \model is perfect at capturing the weaknesses of the graph and has good generalization ability on different defense methods.

For KDD-CUP dataset, besides FGSM, AFGSM and SPEIT, we also include the top 5 candidate attack submissions besides SPEIT. Note that despite SPEIT ranks the 1st in the combined score of attack and defense, it is not the best in attack and teams like u1234 are better in attack. \model outperforms all previous works and significantly reduces the weighted average accuracy over all defense models. 

\subsection{Ablation Studies}

In this section, we analyse in details the performance of \model under different conditions, and how general \model is when we use different surrogate attack models to attack different defense models.

\vpara{Topological Defective Edge Selection.}
In section \ref{sec:gnn-topo} we propose the Topological Defective Edge Selection method. We analysis the effect of this method by illustrating experimental results of different edge selection methods in Figure \ref{fig:edge}(a). "Uniform",  which connects injected nodes with nodes on the test set uniformly, is the most common strategy used by KDD-CUP candidates. Under "Uniform" method, each node in the target set receives the same number of links to the injected nodes. "Random" refers to randomly assigning links between target nodes and injected nodes. As displayed, the Topological Defective Edge Selection does contributes a lot to the attack performance.

\begin{figure}
    \centering
    \mbox
    {
    \begin{subfigure}[Different Edge Selection Methods]{
        \centering
         \includegraphics[width=0.5\linewidth]{figures/edge_selection.png}   
         }
    \end{subfigure}
    \hspace{-0.1in}
    \begin{subfigure}[Different Optimization Methods]{
        \centering
         \includegraphics[width=0.5\linewidth]{figures/smooth.png}   
         }
    \end{subfigure}
    \hspace{-0.1in}
    }
    \caption{Left:Performance of different edge selection methods on KDD-CUP dataset based on smooth feature optimization. Right: Comparison of Smooth Adversarial Optimization and inverse KL-divergence minimization on KDD-CUP dataset.}
    \label{fig:edge}
\end{figure}

\vpara{Smooth Adversarial Optimization.}
The Smooth Adversarial Optimization, proposed in section \ref{sec:smooth}, also has its own advantages. Figure \ref{fig:edge} (b) shows the results of \model and FGSM/AFGSM with/without smooth adversarial optimization. The Smooth Adversarial Optimization prevents gradient loss and contributes a little to the performance of the attack under all three methods.


\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/basemodel.png}
    \caption{\model weighted average on KDD-CUP dataset using different surrogate models for attack. GCN yields the best result. }
    \label{fig:basemodel}
\end{figure}

\vpara{Attack Based on Different Models.}
Despite \model works well when using GCN as surrogate model, how does it work with other surrogate models? Figure \ref{fig:basemodel} illustrates the \model using different models as base models. An interesting result is that GCN turns out to be the best surrogate model if being used during the attack phase. 
\begin{figure}
    \centering
	\includegraphics[width=0.5\textwidth]{figures/heatmap.png}
    \caption{\name generalization across different models with 500 injected nodes. Deeper color suggests more performance reduction. Using surrogate models for attack, and evaluate on target models. Darker color suggests a larger performance reduction. Left: Confusion matrix on KDD-CUP, Right: Confusion matrix on ogbn-arxiv. }
    \label{fig:conf}
\end{figure}

Moreover, Figure \ref{fig:conf} offers visualization for generalization of \model on KDD-CUP and ogb-arxiv dataset with 500 injected nodes. The heat-map shows \model works despite any surrogate attack model we choose, and generalizes to any defense GNN model listed in this paper, despite the scale of generalization may vary.

RobustGCN is a little more robust as defense models, as it is designed to be a more robust GNN against adversarial attacks. On the other hand, GCN yields better attacks. A probable explanation may be that most of the GNN variants are designed based on GCN, making them more similar to GCN. Therefore, their defense may be more easily generalized to by attacks using GCN as surrogate models.

\begin{figure}
    
    \centering
    
	\mbox
	{
		\hspace{-0.1in}
		\begin{subfigure}[TDGIA vs. FGSM  on ogbn-arxiv]{
				\centering
				\includegraphics[width = 0.5 \linewidth]{figures/injection_num_arxiv_2.png}
			}
		\end{subfigure}
        \hspace{-0.1in}
		\begin{subfigure}[TDGIA vs. FGSM on KDD-CUP Data]{
				\centering
				\includegraphics[width = 0.5 \linewidth]{figures/injection_num_aminer_2.png}
			}
		\end{subfigure}
	}
	\mbox
	{
		\hspace{-0.1in}
		%\hfill
		\begin{subfigure}[TDGIA on Different Defense Models\\ on ogbn-arxiv ]{
				\centering
				\includegraphics[width = 0.5 \linewidth]{figures/injection_num_arxiv_1.png}
			}
		\end{subfigure}
		\hspace{-0.1in}
		%\hfill
		\begin{subfigure}[TDGIA on Different Defense Models \\on KDD-CUP Data]{
				\centering
				\includegraphics[width = 0.5 \linewidth]{figures/injection_num_aminer_1.png}
			}
		\end{subfigure}
	}
	\vspace{-0.1in}
    \caption{\model under different numbers of injected nodes. 
  %  (a) \& (b): ogb-arxiv dataset.
  %  (c) \& (d): KDD-CUP 2020 dataset.
  %  (a) \& (c).: Weighted Average Performance of TDGIA and FGSM, performance on KDD-CUP dataset is also evaluated based on the same 7 defense models as ogb-arxiv. 
  %  (b,d).: Performance of different defense models against \model .  
  }
  \vspace{-0.1in}
    \label{fig:diff_injection}
\end{figure}

%\yx{i changed the order of the subfigures in Figure 6, please check and fix the text}\xz{checked}

\vpara{Magnitude of Injection.}
Figure \ref{fig:diff_injection} illustrates the performance curve of FGSM and \model on a weighted average basis, as well as the performance of different defense models under \model as we increase the number of injected nodes on ogbn-arxiv and KDD-CUP datasets from 0 to more than 2000. Some KDD-CUP defense submissions don't support injected nodes being more than 500. As a result, in Figure \ref{fig:diff_injection} we evaluate on KDD-CUP dataset based on the weighted average performance of the same 7 defense models as ogb-arxiv. 

As displayed, \model outperforms the FGSM baseline significantly however the magnitude of injection. Defense models on both KDD-CUP and ogbn-arxiv dataset performs very badly when we expand the number of injected nodes to more than 2000. However, that is still less than $5\%$ the size of the target node sets, or $1.4\%$(for ogbn-arxiv)/$0.4\%$(for KDD-CUP) the size of the whole graph. This emphasis our belief that most GNN models are quite vulnerable towards \model. 

For defense models, RobustGCN performs the best on ogbn-arxiv, while SGCN outperforms all other models on KDD-CUP. The difference of relative performance of different models on different datasets suggests that the robustness of different defense models may depend not only on the model itself and the attack method, but also heavily on the properties of the dataset.  



==> conc.tex <==
In this work, we explore deeply into the graph injection attack (GIA) problem and present the TDGIA attack method. 
TDGIA consists of two modules: the topological defective edge selection for injecting nodes and smooth adversarial optimization for generating features of injected nodes. 
TDGIA achieves the best attack performance in attacking a variety of defense GNN models, compared with various baseline attack methods including the champion solution of KDD-CUP 2020. 
It is also worth mentioning that with only a few number of injected nodes, TDGIA is able to effectively attack GNNs under the black-box and evasion settings. 

In this work, we mainly focus on leveraging the first level neighborhood on the graph to design the attack strategies. 
In the future, we would like to involve higher levels of neighborhood information for advanced attacks. 
Another interesting finding is that among all the GNN variants, using GCN as the surrogate model achieves the best results. 
Further studies on this observation may deepen our understandings of how different GNN variants work, and thus inspire more effective attack designs. 

We continue our research on graph robustness issues and published Graph Robustness Benchmark on NeurIPS 2021. The work is called \textit{Graph Robustness Benchmark: Benchmarking the Adversarial Robustness of Graph Machine Learning}(GRB) and we also created a website for attack and defense submissions, see GRB.\footnote{\url{https://cogdl.ai/grb/home}}



==> removed_tables.tex <==
\iffalse
\xz{The below tables can be replaced by figures}
\begin{table*}[t]
\small
    \centering
    \caption{ Performance of GIA on KDD-CUP dataset, attack based on different edge selection methods.  }
    
    \label{tab:edge seclections}
    % \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline \hline
       Edge selection Method  & Average Accuracy(\%) & Top-3 Defense(\%) & Weighted Average (\%) &  Reduction(\%) \\
       \hline
       Clean & 65.54 & 70.02 & 68.57 & -\\
       \hline
     uniform & 59.26 & 67.71 & 65.29 & 3.28\\
      random & 58.45 & 67.13 & 64.43 & 4.14 \\
       Topological Defective & \textbf{55.00} & \textbf{64.49} & \textbf{60.49} & \textbf{8.08} \\
     
      % \cline{2-6}
       
      % &Mixed& \textbf{54.80}&65.73 & 61.04 & 7.53 \\
      % & \multicolumn{5}{c|}{\xz{Shall we remove the "mixed"? It seems that mixed attack is worse than attack only on GCN}}\\
        \hline \hline
    \end{tabular}
   
\end{table*}
\fi
\iffalse
\begin{table*}[t]
\small
    \centering
    \caption{ Performance of GIA on KDD-CUP dataset, attack based on different base models, and evaluated on KDD-CUP top defense submissions. Best results are bolded.}
    
    \label{tab:basemodel}
    % \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline \hline
       Method &Base model & Average Accuracy(\%) & Top-3 Defense(\%) & Weighted Average (\%) &  Reduction(\%) \\
       \hline
       Clean & - & 65.54 & 70.02 & 68.57 & -\\
       \hline
       \multirow{7}*{\makecell{\model}}&RobustGCN &57.24 & 65.83 & 62.53 & 6.04\\
       &sgcn & 58.01 & 66.28 & 62.88 & 5.69\\
       &tagcn & 58.35 & 65.82 & 62.90 & 5.67\\
       &GCN & \textbf{55.00} & \textbf{64.49} & \textbf{60.49} & \textbf{8.08} \\
       &GIN & 56.83 & 65.70 & 62.15 & 6.42 \\
       &GraphSAGE & 59.35 & 66.43 & 63.70 & 4.87 \\
       & appnp & 55.80 & 65.93 & 61.76 & 6.81\\
      % \cline{2-6}
       
      % &Mixed& \textbf{54.80}&65.73 & 61.04 & 7.53 \\
      % & \multicolumn{5}{c|}{\xz{Shall we remove the "mixed"? It seems that mixed attack is worse than attack only on GCN}}\\
        \hline \hline
    \end{tabular}
   
\end{table*}

\begin{table*}[t]
\small
    \centering
    \caption{ Performance of GIA on ogb-arxiv dataset, using different number of attack nodes \xz{Better make a figure of this}}
    
    \label{tab:numbernode}
    % \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline \hline
       Method &Attack Nodes & Average Accuracy(\%) & Top-3 Defense(\%) & Weighted Average (\%) &  Reduction(\%) \\
       \hline
       Clean & - & 70.86 & 71.61 & 71.34 & -\\
       \hline
       \multirow{10}*{\makecell{\model}}& 250 &62.35 & 63.84 & 63.44 & 7.90\\
       &500 & 57.00 & 59.23 & 58.53 & 12.81\\
       &750 & 52.42 & 55.08 & 54.22 & 17.12\\
       &1000& 43.94 & 50.54 & 48.37 & 22.97 \\
       &1250 & 37.07 & 45.95 & 42.91 & 28.43 \\
       &1500 & 29.91 & 41.30 & 37.08 & 34.26 \\
       & 1750 & 22.12 & 35.81 & 30.82 & 40.52\\
       & 2000 & 16.56 & 30.23 & 25.34 & 46.00\\
       & 2250 & 12.89 & 23.69 & 20.47 & 50.87\\
       & \multicolumn{5}{c|}{\xz{shall we compare with FGSM?Which dataset shall we use?}} \\ 
      % \cline{2-6}
       
      % &Mixed& \textbf{54.80}&65.73 & 61.04 & 7.53 \\
      % & \multicolumn{5}{c|}{\xz{Shall we remove the "mixed"? It seems that mixed attack is worse than attack only on GCN}}\\
        \hline \hline
    \end{tabular}
   
\end{table*}
\fi

\iffalse
\xz{original table here:}
\begin{table*}[t]
\small
    \centering
    \caption{ Performance on KDD-CUP dataset. Best results are bolded.}
    \vspace{-0.1in}
    \label{tab:kddcup}
    % \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline \hline
       & Attack Method/Base Model & Average Accuracy(\%) & Top-3 Defense(\%) & Weighted Average (\%) &  Reduction(\%) \\
       \cline{1-6}
      Clean & - & 65.54 & 70.02 & 68.57 & -\\
       \hline
       %&NTTDOCOMO LABS& 52.00$\pm$0.97 & 13.91\%\\
      %& ADVERSARIES & 44.85$\pm$1.39 & 25.91\%\\
      % & DeepBlueAI & 42.14$\pm$3.10 &30.23\%\\
      % & cccn & 52.01$\pm$0.97 \\
      \multirow{28}*{\makecell{ Competition\\ Submissions}}  & ADVERSARIES& 63.44 &68.85 &67.09 & 1.48\\
       %& zmzyczfy & 36.63$\pm$2.88\\
       & DAFTSTONE & 63.91 &68.50 & 67.02 & 1.55 \\
       & DeepBlueAI & 61.44 & 69.4 & 67.26 & 1.31\\
       & Dminers & 63.76 & 69.39 & 67.48 & 1.09\\
       &Fengari & 63.78 & 69.41 & 67.45 & 1.12\\
       &GraphOverflow& 63.75& 69.34& 67.44 & 1.13\\
       &MSUPSUDSE&65.49   &  69.97  &  68.52 & 0.05\\
       &NTTDOCOMOLABS &60.21 & 68.80 & 66.27 & 2.30 \\
       & Neutrino & 63.62 &69.42 &67.42 & 1.15\\
       & RunningZ & 63.96 & 69.40 & 67.55 & 1.02 \\
       & SPEIT-submission & 61.97 & 69.49 & 67.32 & 1.25\\
       & Selina& 64.67& 69.40& 67.79 & 0.78\\
       & TSAIL & 63.90 & 69.40 & 67.55 & 1.02 \\
       & cccn & 63.11 & 69.26 & 67.28 & 1.29 \\
       &darkhorse  &     63.94     &          69.33      &   67.51 & 1.06\\
&kaige  &         63.90   &            69.41    &     67.49 & 1.08\\
&idvl   &         63.57   &            69.42    &     67.39 & 1.18\\
&hhhvjk   &       65.00   &            69.38   &      67.93 & 0.64\\
&fashui01  &      63.69    &           69.42  &       67.42 & 1.15\\
&shengz     &     63.99     &          69.40   &      67.55 & 1.02\\
&sc        &      64.48    &           69.11     &    67.41 & 1.16\\
&simongeisler   & 60.02     &    68.59  &       66.29 & 2.28\\
&tofu     &       63.87  &             69.39  &       67.50 & 1.07\\
&yama     &       64.21   &            68.77  &       67.23 & 1.34\\
&yaowenxi    &    63.94   &            69.33    &     67.50& 1.07\\
&tzpppp   &       65.01       &        69.38    &     67.94 & 0.63\\
&u1234x1234 &     61.18     &          67.95 &  64.87 & 3.70\\
&zhangs    &      63.73      &         69.43   &      67.51 & 1.06\\
       \hline
        \multirow{3}*{\makecell{Baseline \\Methods}}&FGSM & 59.80 & 67.44 & 65.04 & 3.53 \\
      %  &FGSM(use sin)& 58.49 & 67.09 & 64.44 & 4.13\\
      & AFGSM & 59.22 & 67.37 & 64.74 & 3.83\\
%       & AFGSM(use sin) & 58.43 & 67.05 & 64.39 & 4.18\\
       & SPEIT & 61.89 & 68.16 & 66.13 & 2.44 \\
       \hline
       & Best of Above & 59.22 & 67.37 & 64.74 & 3.83\\
       \hline\hline
       \multirow{7}*{\makecell{GIA \\ with different \\ base models}}&RobustGCN &57.24 & 65.83 & 62.53 & 6.04\\
       &sgcn & 58.01 & 66.28 & 62.88 & 5.69\\
       &tagcn & 58.35 & 65.82 & 62.90 & 5.67\\
       &GCN & \textbf{55.00} & \textbf{64.49} & \textbf{60.49} & \textbf{8.08} \\
       &GIN & 56.83 & 65.70 & 62.15 & 6.42 \\
       &GraphSAGE & 59.35 & 66.43 & 63.70 & 4.87 \\
       & appnp & 55.80 & 65.93 & 61.76 & 6.81\\
      % \cline{2-6}
       
      % &Mixed& \textbf{54.80}&65.73 & 61.04 & 7.53 \\
      % & \multicolumn{5}{c|}{\xz{Shall we remove the "mixed"? It seems that mixed attack is worse than attack only on GCN}}\\
        \hline \hline
    \end{tabular}
    \vspace{-0.15in}
\end{table*}

\begin{table*}[t]
\small
    \centering
    \caption{ Performance of GIA on ogb-arxiv dataset. Best results are bolded.\xz{Do we still need "different base models"?}
    }
    \label{tab:ogb}
    % \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline \hline
       & Attack Method/Base Model & Average Accuracy(\%) & Top-3 Defense(\%) & Weighted Average (\%) &  Reduction(\%) \\
       \cline{1-6}
      Clean & - & 70.86 & 71.61 & 71.34 & -\\
       \hline
       %&NTTDOCOMO LABS& 52.00$\pm$0.97 & 13.91\%\\
      %& ADVERSARIES & 44.85$\pm$1.39 & 25.91\%\\
      % & DeepBlueAI & 42.14$\pm$3.10 &30.23\%\\
      % & cccn & 52.01$\pm$0.97 \\
     
       \hline
        \multirow{3}*{\makecell{Baseline \\Methods}}&FGSM&66.40 & 69.57 & 68.62 & 2.72 \\
       & AFGSM & 62.60 & 69.08 & 66.96 & 4.38\\
       & SPEIT & 66.93 & 69.56 & 68.63 & 2.71 \\
       
       \hline\hline
       \multirow{7}*{\makecell{GIA \\ with different \\ base models}}&RobustGCN & 59.21 & 63.81 & 61.90 & 9.44\\
       &sgcn & 61.50 & 64.94 & 63.68 & 7.66\\
       &tagcn & 57.47 & 61.61 & 60.33 & 11.01\\
       &GCN & 57.00 & \textbf{59.23} & \textbf{58.53} & \textbf{12.81} \\
       &GIN & 60.13 & 64.35 & 62.80 & 8.54\\
       &GraphSAGE & 60.92 &  63.86 & 62.82 & 8.52\\
       & appnp & \textbf{55.90} & 62.87 & 60.32 & 11.02\\
      % \cline{2-6}
       
      % &Mixed& \textbf{54.80}&65.73 & 61.04 & 7.53 \\
      % & \multicolumn{5}{c|}{\xz{Shall we remove the "mixed"? It seems that mixed attack is worse than attack only on GCN}}\\
        \hline \hline
    \end{tabular}
    \vspace{-0.15in}
\end{table*}
\hide{
\begin{table*}[t]
\small
    \centering
    \caption{ Performance of GIA on reddit dataset. Best results are bolded.}
    \vspace{-0.1in}
    \label{tab:reddit}
    % \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline \hline
       & Attack Method/Base Model & Average Accuracy(\%) & Top-3 Defense(\%) & Weighted Average (\%) &  Reduction(\%) \\
       \cline{1-6}
      Clean & - & 94.86 & 95.94 & 95.62 & -\\
       \hline
       %&NTTDOCOMO LABS& 52.00$\pm$0.97 & 13.91\%\\
      %& ADVERSARIES & 44.85$\pm$1.39 & 25.91\%\\
      % & DeepBlueAI & 42.14$\pm$3.10 &30.23\%\\
      % & cccn & 52.01$\pm$0.97 \\
     
       \hline
        \multirow{3}*{\makecell{Baseline \\Methods}}&FGSM& 92.26 & 94.61 & 93.80 & 1.82\\
       & AFGSM & 91.46 & 94.64 & 93.61 & 2.01\\
       & SPEIT & 93.35 & 94.27 & 93.99 & 1.63\\ 
       
       \hline\hline
       \multirow{7}*{\makecell{GIA \\ with different \\ base models}}&RobustGCN & 86.73 & 89.49 & 88.51 & 7.11\\
       &sgcn & 87.15 & 91.67 & 89.78 & 5.84\\
       &tagcn &\textbf{80.89} & 89.08 & \textbf{86.79} & \textbf{8.83}\\
       &GCN & 86.11 & \textbf{88.95} & 88.14 & 7.48 \\
       &GIN & 86.02 & 89.34 & 88.42 & 7.20\\
       &GraphSAGE & 89.94 &91.28 & 90.79 & 4.83\\
       & appnp & 81.08 & 89.77 & 87.22 & 8.40 \\
      % \cline{2-6}
       
      % &Mixed& \textbf{54.80}&65.73 & 61.04 & 7.53 \\
      % & \multicolumn{5}{c|}{\xz{Shall we remove the "mixed"? It seems that mixed attack is worse than attack only on GCN}}\\
        \hline \hline
    \end{tabular}
   
\end{table*}
}
\fi

\hide{
\xz{Actually simply randomize the "level-2 perturbation" doesn't make things much worse. Shall we just remove the next section?}

Most of these ways to generate $w_{u,1}$ only incorporates the feature or degree information of node $u$ and $v$, and does not correlate to $w_{t,i},t\neq u$. That is to say, we can separate $\sum_{u\in \mathcal{A}_1(v)\backslash\mathcal{A}_1(v)} w_{u,1}$ and $\sum_{u\in \mathcal{A}_1(v)} w_{u,1}$. 

Take $c_1=\sum_{u\in \mathcal{A}_1(v)\backslash\mathcal{A}_1(v)} w_{u,1}$, and $c_2=\sum_{u\in \mathcal{A}_1(v)} w_{u,1}$, then $r_{v,1}=\frac{c_1}{c_1+c_2}=\frac{1}{1+\frac{c_2}{c_1}}$, given $c_1$ does not change due to $c_2$, this suggests us that, to make $\sum r_{v,1}$ large, the injected nodes shall be connected to nodes with $\lambda=\frac{c_1}{c_2}$ being large. Here $c_2$ can be approximated using equation \ref{eqn:w1} and \ref{eqn:w2}. 
\xz{needs refinement}


\vpara{Maximization of level-2 perturbation}
\xz{maximizing level-1 and level-2 perturbation follows different logic, which is hard to describe.}

Suppose we're already maximizing $\sum_{v\in C}r_{v,1}$ by assigning the injection nodes to nodes in $C$ with minimal $c_2$.

As every injection node may be limited to a certain number of links to avoid being detected and removed by defense methods, assigning those links still remain a question, as two nodes that are linked to the same injection node becomes second-level neighbors of each other, and start to influence the embeddings of each other.

We start from maximizing $\sum_{v\in C} r_{v,2}$, still it's better to add neighbors to those nodes with a small $c_2=\sum_{u\in \mathcal{A}_2(v) w_{u,2}}$, however that is already achieved in the level-1 perturbation part. 

Recall equation (\ref{attackrule}),

\beq{
\Delta \mathbf{h}_{v}^f=\sum_i\sum_{u\in \mathcal{A}'_i(v)} \Delta w_{u,i}\sum_{l=1}^{f}\mathbf{p}_{il}\mathbf{h}_u^{l-1}
}

For $i=2$, we tend to maximize the scale of 

\beq{
\Delta \mathbf{h}_{v}^\mathbf{f}(2)=\sum_{u\in \mathcal{A}'_2(v)} \Delta w_{u,2}\sum_{l=1}^{f}\mathbf{p}_{2l}\mathbf{h}_u^{l-1}
}

\xz{ This is just a logical way, needs refinement on this expression}
Different from newly injected nodes whose embeddings are easy to adjust, for level-2 perturbation, the nodes that newly appear in second-level neighborhood are usually nodes that are linked together by an injection node. And their $\mathbf{h}_u$ are fixed as we cannot change features of existing nodes in GIA. 

This means it is better to make the newly-introduced nodes far-away from the original representation. That is to say, we shall let 

\beq{
\begin{split}
d_1=\frac{\sum_{u\in A_2(v)}  w_{u,2}\sum_{l=1}^{f}\mathbf{p}_{2l}\mathbf{h}_u^{l-1}}{\sum_{u\in  A_2(v)}w_{u,2}}
\\d_2=\frac{\sum_{u\in \mathcal{A}'_2(v)\backslash A_2(v)}  w_{u,2}\sum_{l=1}^{f}\mathbf{p}_{2l}\mathbf{h}_u^{l-1}}{\sum_{u\in \mathcal{A}'_2(v)\backslash A_2(v)}w_{u,2}}
\end{split}
}

be as different as possible. Which means for GIA it's more efficient to link nodes with different $\mathbf{h}_u^{l}$ to the same injection node. That is to say, make $||d_1-d_2||$ as large as possible. 


\xz{ Is it really needed?}

}

\hide{
\begin{table*}[t]
\small
    \centering
    \caption{ Performance of using inverse cross entropy directly/ using smooth feature optimization on FGSM, AFGSM and \model  on Aminer dataset. Using GCN as base model.}
    \label{tab:sm}
    % \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline \hline
        Attack Method & Optimization & Average Accuracy(\%) & Top-3 Defense(\%) & Weighted Average (\%) &  Reduction(\%) \\
       \cline{1-6}
       Clean& & 65.54 & 70.02 & 68.57 & -\\
       \hline
       %&NTTDOCOMO LABS& 52.00$\pm$0.97 & 13.91\%\\
      %& ADVERSARIES & 44.85$\pm$1.39 & 25.91\%\\
      % & DeepBlueAI & 42.14$\pm$3.10 &30.23\%\\
      % & cccn & 52.01$\pm$0.97 \\
     
       \hline\hline
        \multirow{2}*{FGSM} & Inverse KL &59.80 & 67.44 & 65.04 & 3.53 \\
        & Smooth Opt & 58.45 & 67.13 & 64.43 & 4.14 \\
        \hline
       \multirow{2}*{AFGSM} & Inverse KL & 59.22 & 67.37 & 64.74 & 3.83\\
       & Smooth Opt & 58.52 & 67.15 & 64.48 & 4.09\\
       \hline\hline
       \multirow{2}*{\model} & Inverse KL & \textbf{54.58} & 65.72 & 60.85 & 7.72\\
       & Smooth Opt & 55.00 & \textbf{64.49} & \textbf{60.49} & \textbf{8.08}\\
      % \cline{2-6}
       
      % &Mixed& \textbf{54.80}&65.73 & 61.04 & 7.53 \\
      % & \multicolumn{5}{c|}{\xz{Shall we remove the "mixed"? It seems that mixed attack is worse than attack only on GCN}}\\
        \hline \hline
    \end{tabular}
    \vspace{-0.15in}
\end{table*}
}
